The Self-Improvement Paradox: Can Language Models Bootstrap Reasoning Capabilities without External Scaffolding?

Self-improving large language models (LLMs) -- i.e., to improve the performance of an LLM by fine-tuning it with synthetic data generated by itself -- is a promising way to advance the capabilities of LLMs while avoiding extensive supervision. Existing approaches to self-improvement often rely on external supervision signals in the form of seed data and/or assistance from third-party models. This paper presents Crescent -- a simple yet effective framework for generating high-quality synthetic question-answer data in a fully autonomous manner. Crescent first elicits the LLM to generate raw questions via a bait prompt, then diversifies these questions leveraging a rejection sampling-based self-deduplication, and finally feeds the questions to the LLM and collects the corresponding answers by means of majority voting. We show that Crescent sheds light on the potential of true self-improvement with zero external supervision signals for math reasoning; in particular, Crescent-generated question-answer pairs suffice to (i) improve the reasoning capabilities of an LLM while preserving its general performance (especially in the 0-shot setting); and (ii) distil LLM knowledge to weaker models more effectively than existing methods based on seed-dataset augmentation.

==> macros.tex <==
% !TEX root = ./main.tex
%
\RequirePackage{todonotes}

\newcommand{\cmscomment}[1]{\todo[color=blue!10,size=\small,fancyline,author=CMS]{#1}\xspace}
\newcommand{\cmscommentinline}[1]{\todo[inline,color=blue!10,author=CMS]{#1}\xspace}
\newcommand{\atcms}{\colorbox{blue!10}{\textbf{@CMS}}}

\newcommand{\sytcomment}[1]{\todo[color=green!10,size=\small,fancyline,author=SYT]{#1}\xspace}
\newcommand{\sytcommentinline}[1]{\todo[inline,color=green!10,author=SYT]{#1}\xspace}
\newcommand{\atsyt}{\colorbox{green!10}{\textbf{@SYT}}}

\newcommand{\promptfont}[1]{\mathsf{#1}\vphantom{y}}
\newcommand{\promptColor}[1]{\textcolor{NavyBlue}{\mathsf{#1}\vphantom{y}}}

\newcommand{\langname}{\textsc{Crescent}\xspace}

\newcommand{\green}[1]{\textcolor{ForestGreen}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\nblue}[1]{\textcolor{NavyBlue}{#1}}
\newcommand{\red}[1]{\textcolor{Red}{#1}}
\newcommand{\orange}[1]{\textcolor{RedOrange}{#1}}
\newcommand{\gray}[1]{\textcolor{Gray}{#1}}
\newcommand{\maroon}[1]{\textcolor{Maroon}{#1}}
\newcommand{\violet}[1]{\textcolor{Violet}{#1}}

\DeclarePairedDelimiter\norm{\lVert}{\rVert}
\newcommand{\defeq}{{}\triangleq{}}
\newcommand{\ddefeq}{\ {}\defeq{}\ }
\newcommand{\eeq}{~{}={}~}

==> sections/Acknowledgements.tex <==
\section*{Acknowledgments}
